Trellis-Based Equalization for Sparse ISI Channels Revisited

Sparse intersymbol-interference (ISI) channels are encountered in a variety of high-data-rate communication systems. Such channels have a large channel memory length, but only a small number of significant channel coefficients. In this paper, trellis-based equalization of sparse ISI channels is revisited. Due to the large channel memory length, the complexity of maximum-likelihood detection, e.g., by means of the Viterbi algorithm (VA), is normally prohibitive. In the first part of the paper, a unified framework based on factor graphs is presented for complexity reduction without loss of optimality. In this new context, two known reduced-complexity algorithms for sparse ISI channels are recapitulated: The multi-trellis VA (M-VA) and the parallel-trellis VA (P-VA). It is shown that the M-VA, although claimed, does not lead to a reduced computational complexity. The P-VA, on the other hand, leads to a significant complexity reduction, but can only be applied for a certain class of sparse channels. In the second part of the paper, a unified approach is investigated to tackle general sparse channels: It is shown that the use of a linear filter at the receiver renders the application of standard reduced-state trellis-based equalizer algorithms feasible, without significant loss of optimality. Numerical results verify the efficiency of the proposed receiver structure.

==> Pic/dependencies <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
0 32 #000000
0 33 #dcdcdc
0 34 #b5b5b5
2 1 0 2 0 33 50 0 20 6.000 0 0 -1 0 0 8
	 5850 4725 6120 4725 6120 4950 6300 4950 5985 5175 5670 4950
	 5850 4950 5850 4725
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1710 10575 1710 13275
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 10575 10800 13275
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 11250 2025 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 11250 5535 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 11250 6435 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 3510 11250 3510 12600
2 1 0 2 23 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 11250 6435 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 4635 11250 4635 12600
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3510 11250 7335 12600
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4635 11250 8235 12600
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 11250 9135 12600
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 11250 10305 12600
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1710 5670 1710 8370
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 5670 10800 8370
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 6345 2025 7695
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 6345 5535 7695
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 6345 6435 7695
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 3510 6345 3510 7695
2 1 0 2 11 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 6345 5535 7695
2 1 0 2 23 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 6345 6435 7695
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 4635 6345 4635 7695
2 1 0 2 11 33 50 0 -1 0.000 0 0 -1 0 0 2
	 3510 6345 6435 7695
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4635 6345 7335 7695
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 6345 8235 7695
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 6345 9135 7695
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7335 6345 10305 7695
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3510 6345 7335 7695
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4635 6345 8235 7695
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 6345 9135 7695
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 6345 10305 7695
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5985 12600 2025 11250
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 7335 11250 7335 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 8235 11250 8235 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 9135 11250 9135 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 10305 11250 10305 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 10305 6345 10305 7695
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 9135 6345 9135 7695
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 8235 6345 8235 7695
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 7335 6345 7335 7695
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4185 11250 7785 12600
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5085 11250 8685 12600
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5985 11250 9585 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 11250 2700 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 4185 11250 4185 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 5085 11250 5085 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 5985 11250 5985 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6885 11250 6885 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6885 11250 6885 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 7785 11250 7785 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 8685 11250 8685 12600
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 9585 11250 9585 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3510 11250 6885 12600
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6885 12600 2700 11250
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 11250 6435 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4185 11250 7335 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4635 11250 7785 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5085 11250 8235 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 11250 8685 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5985 11250 9135 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 11250 9585 12600
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6885 11250 10305 12600
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1710 1125 1710 3825
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 1125 10800 3825
2 2 0 2 33 33 51 0 20 0.000 0 0 -1 0 0 5
	 10800 1125 12330 1125 12330 3825 10800 3825 10800 1125
2 2 0 2 33 33 51 0 20 0.000 0 0 -1 0 0 5
	 180 1125 1710 1125 1710 3825 180 3825 180 1125
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 3510 900 3510 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 1 0 2
	3 1 1.00 60.00 120.00
	 2025 900 2025 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 5535 900 5535 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 6435 900 6435 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2340 3690 2340 3870
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 1 0 2
	3 1 1.00 60.00 120.00
	 4185 3780 2385 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 6615 3780 4815 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6660 3690 6660 3870
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6705 3690 6705 3870
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 1 0 2
	3 1 1.00 60.00 120.00
	 8460 3780 6750 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 10665 3780 8955 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 10710 3690 10710 3870
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 1800 2025 3150
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 1800 5535 3150
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 1800 6435 3150
2 1 1 2 0 33 50 0 -1 6.000 0 0 -1 0 0 2
	 3510 1800 3510 3150
2 1 0 2 11 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 1800 5535 3150
2 1 1 2 11 33 50 0 -1 6.000 0 0 -1 0 0 2
	 3510 1800 6435 3150
2 1 0 2 23 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 1800 6435 3150
4 0 0 50 0 0 12 0.0000 2 180 1365 6435 4950 Complete diagram\001
4 1 0 50 0 2 14 0.0000 2 195 270 0 10125 (b)\001
4 1 0 50 0 0 12 0.0000 2 165 465 4185 12915 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4635 12915 $+\\!4$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5085 12915 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5985 12915 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6885 12915 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5535 12915 $+\\!6$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6435 12915 $+\\!8$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8235 12915 $+\\!12$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7335 12915 $+\\!10$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7785 12915 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8685 12915 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9135 12915 $+\\!14$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9585 12915 $+\\!15$\001
4 1 0 50 0 0 12 0.0000 2 195 660 2025 12915 $y[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 2700 12915 $y[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 3510 12915 $y[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 195 1125 10305 12915 $y[k_0\\!+\\!16]$\001
4 1 0 50 0 0 12 0.0000 2 195 1575 2025 11070 $\\underline{x[k_0]}$\001
4 1 0 50 0 0 12 0.0000 2 195 1950 3510 11070 $\\underline{x[k_0\\!+\\!2]}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 4635 11070 $\\underline{+\\!4}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 5535 11070 $\\underline{+\\!6}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 6435 11070 $\\underline{+\\!8}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 8235 11070 $\\underline{+\\!12}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 7335 11070 $\\underline{+\\!10}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 8685 11070 $\\underline{+\\!13}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 9135 11070 $\\underline{+\\!14}$\001
4 1 0 50 0 0 12 0.0000 2 195 2040 10305 11070 $\\underline{x[k_0\\!+\\!16]}$\001
4 1 0 51 0 0 12 0.0000 2 195 1470 9585 11070 $\\underline{+\\!15}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 7785 11070 $\\underline{+\\!11}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 6885 11070 $\\underline{+\\!9}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 5985 11070 $\\underline{+\\!7}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 5085 11070 $\\underline{+\\!5}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 4185 11070 $\\underline{+\\!3}$\001
4 1 0 50 0 0 12 0.0000 2 195 1950 2700 11070 $\\underline{x[k_0\\!+\\!1]}$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4185 8010 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4635 8010 $+\\!4$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5085 8010 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5985 8010 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6885 8010 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5535 8010 $+\\!6$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6435 8010 $+\\!8$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8235 8010 $+\\!12$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7335 8010 $+\\!10$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7785 8010 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8685 8010 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9135 8010 $+\\!14$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9585 8010 $+\\!15$\001
4 1 0 50 0 0 12 0.0000 2 195 660 2025 8010 $y[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 2700 8010 $y[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 3510 8010 $y[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 195 1125 10305 8010 $y[k_0\\!+\\!16]$\001
4 1 0 50 0 0 12 0.0000 2 195 1575 2025 6165 $\\underline{x[k_0]}$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 2700 6165 $x[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1950 3510 6165 $\\underline{x[k_0\\!+\\!2]}$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4185 6165 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 4635 6165 $\\underline{+\\!4}$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5085 6165 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5985 6165 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6885 6165 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 5535 6165 $\\underline{+\\!6}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 6435 6165 $\\underline{+\\!8}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 8235 6165 $\\underline{+\\!12}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 7335 6165 $\\underline{+\\!10}$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7785 6165 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8685 6165 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 9135 6165 $\\underline{+\\!14}$\001
4 1 0 50 0 0 12 0.0000 2 195 2040 10305 6165 $\\underline{x[k_0\\!+\\!16]}$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9585 6165 $+\\!15$\001
4 1 0 50 0 2 14 0.0000 2 195 255 0 0 (a)\001
4 0 0 50 0 0 14 0.0000 2 210 8055 270 10125 CIR $\\;\\mathbf{h}^{(2)} = [\\,h_0\\;\\; 0 \\;\\; 0 \\;\\; 0 \\;\\; 0 \\;\\; 0 \\;\\; 0 \\;\\; h_1 \\;\\;h_{2} \\,]^{\\rm T}$\001
4 0 0 50 0 0 14 0.0000 2 210 8010 270 0 CIR $\\;\\mathbf{h}^{(1)} = [\\,h_0\\;\\; 0 \\;\\; 0 \\;\\; 0 \\;\\; 0 \\;\\; 0 \\;\\; h_1 \\;\\; 0\\;\\;h_{2} \\,]^{\\rm T}$\001
4 1 0 50 0 0 12 0.0000 2 135 765 900 2070 Decisions\001
4 1 0 50 0 0 12 0.0000 2 195 1770 900 2430 $\\hat{x}[\\,.\\,]\\;$ already\001
4 1 0 50 0 0 12 0.0000 2 135 675 900 2790 available\001
4 1 0 50 0 0 12 0.0000 2 135 960 11565 2250 No influence\001
4 1 0 50 0 0 12 0.0000 2 195 1410 11565 2610 of $\\tilde{x}[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4185 3465 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4635 3465 $+\\!4$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5085 3465 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5985 3465 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6885 3465 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5535 3465 $+\\!6$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6435 3465 $+\\!8$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8235 3465 $+\\!12$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7335 3465 $+\\!10$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7785 3465 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8685 3465 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9135 3465 $+\\!14$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9585 3465 $+\\!15$\001
4 1 0 50 0 0 12 0.0000 2 195 660 2025 3465 $y[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 2700 3465 $y[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 3510 3465 $y[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 195 1125 10305 3465 $y[k_0\\!+\\!16]$\001
4 1 0 50 0 0 12 0.0000 2 195 660 2025 1620 $x[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 2700 1620 $x[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 3510 1620 $x[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4185 1620 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4635 1620 $+\\!4$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5085 1620 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5985 1620 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6885 1620 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5535 1620 $+\\!6$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6435 1620 $+\\!8$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8235 1620 $+\\!12$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7335 1620 $+\\!10$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7785 1620 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8685 1620 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9135 1620 $+\\!14$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9585 1620 $+\\!15$\001
4 1 0 50 0 0 12 0.0000 2 195 1125 10305 1620 $x[k_0\\!+\\!16]$\001
4 1 0 50 0 0 12 0.0000 2 195 1215 2025 765 $\\tilde{x}[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1500 3510 765 $\\hat{x}[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 195 1500 5535 765 $\\hat{x}[k_0\\!+\\!6]$\001
4 1 0 50 0 0 12 0.0000 2 195 1500 6435 765 $\\hat{x}[k_0\\!+\\!8]$\001
4 1 0 50 0 0 12 0.0000 2 165 285 4500 3870 $L$\001
4 1 0 50 0 0 12 0.0000 2 165 285 8685 3870 $L$\001


==> Pic/dependencies_ISIT <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
0 32 #000000
0 33 #dcdcdc
0 34 #b5b5b5
6 5625 4275 15750 7065
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6120 4320 6120 7020
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 15210 4320 15210 7020
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 4995 6435 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 9945 4995 9945 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 10845 4995 10845 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 7920 4995 7920 6345
2 1 0 2 11 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 4995 9945 6345
2 1 0 2 23 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 4995 10845 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 9045 4995 9045 6345
2 1 0 2 11 33 50 0 -1 0.000 0 0 -1 0 0 2
	 7920 4995 10845 6345
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9045 4995 11745 6345
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9945 4995 12645 6345
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10845 4995 13545 6345
2 1 0 2 11 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11745 4995 14715 6345
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7920 4995 11745 6345
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9045 4995 12645 6345
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9945 4995 13545 6345
2 1 0 2 23 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10845 4995 14715 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 14715 4995 14715 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 13545 4995 13545 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 12645 4995 12645 6345
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 11745 4995 11745 6345
4 1 0 50 0 0 12 0.0000 2 165 465 8595 6660 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 165 465 9045 6660 $+\\!4$\001
4 1 0 50 0 0 12 0.0000 2 165 465 9495 6660 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 10395 6660 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 11295 6660 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 165 465 9945 6660 $+\\!6$\001
4 1 0 50 0 0 12 0.0000 2 165 465 10845 6660 $+\\!8$\001
4 1 0 50 0 0 12 0.0000 2 165 555 12645 6660 $+\\!12$\001
4 1 0 50 0 0 12 0.0000 2 165 555 11745 6660 $+\\!10$\001
4 1 0 50 0 0 12 0.0000 2 165 555 12195 6660 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 13095 6660 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 165 555 13545 6660 $+\\!14$\001
4 1 0 50 0 0 12 0.0000 2 165 555 13995 6660 $+\\!15$\001
4 1 0 50 0 0 12 0.0000 2 195 660 6435 6660 $y[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 7110 6660 $y[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 7920 6660 $y[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 195 1125 14715 6660 $y[k_0\\!+\\!16]$\001
4 1 0 50 0 0 12 0.0000 2 195 1575 6435 4815 $\\underline{x[k_0]}$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 7110 4815 $x[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1950 7920 4815 $\\underline{x[k_0\\!+\\!2]}$\001
4 1 0 50 0 0 12 0.0000 2 165 465 8595 4815 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 9045 4815 $\\underline{+\\!4}$\001
4 1 0 50 0 0 12 0.0000 2 165 465 9495 4815 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 10395 4815 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 11295 4815 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 9945 4815 $\\underline{+\\!6}$\001
4 1 0 50 0 0 12 0.0000 2 195 1380 10845 4815 $\\underline{+\\!8}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 12645 4815 $\\underline{+\\!12}$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 11745 4815 $\\underline{+\\!10}$\001
4 1 0 50 0 0 12 0.0000 2 165 555 12195 4815 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 13095 4815 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 195 1470 13545 4815 $\\underline{+\\!14}$\001
4 1 0 50 0 0 12 0.0000 2 195 2040 14715 4815 $\\underline{x[k_0\\!+\\!16]}$\001
4 1 0 50 0 0 12 0.0000 2 165 555 13995 4815 $+\\!15$\001
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1710 1125 1710 3825
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 1125 10800 3825
2 2 0 2 33 33 51 0 20 0.000 0 0 -1 0 0 5
	 10800 1125 12330 1125 12330 3825 10800 3825 10800 1125
2 2 0 2 33 33 51 0 20 0.000 0 0 -1 0 0 5
	 180 1125 1710 1125 1710 3825 180 3825 180 1125
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 3510 900 3510 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 1 0 2
	3 1 1.00 60.00 120.00
	 2025 900 2025 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 5535 900 5535 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 6435 900 6435 1395
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2340 3690 2340 3870
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 1 0 2
	3 1 1.00 60.00 120.00
	 4185 3780 2385 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 6615 3780 4815 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6660 3690 6660 3870
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6705 3690 6705 3870
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 1 0 2
	3 1 1.00 60.00 120.00
	 8460 3780 6750 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 1 2
	3 1 1.00 60.00 120.00
	 10665 3780 8955 3780
2 1 0 1 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 10710 3690 10710 3870
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 1800 2025 3150
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 5535 1800 5535 3150
2 1 0 2 0 33 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 1800 6435 3150
2 1 1 2 0 33 50 0 -1 6.000 0 0 -1 0 0 2
	 3510 1800 3510 3150
2 1 0 2 11 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 1800 5535 3150
2 1 1 2 11 33 50 0 -1 6.000 0 0 -1 0 0 2
	 3510 1800 6435 3150
2 1 0 2 23 33 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 1800 6435 3150
2 1 0 2 0 33 50 0 20 6.000 0 0 -1 0 0 8
	 4410 5895 4410 5625 4635 5625 4635 5445 4860 5760 4635 6075
	 4635 5895 4410 5895
4 1 0 50 0 0 12 0.0000 2 135 765 900 2070 Decisions\001
4 1 0 50 0 0 12 0.0000 2 195 1770 900 2430 $\\hat{x}[\\,.\\,]\\;$ already\001
4 1 0 50 0 0 12 0.0000 2 135 960 11565 2250 No influence\001
4 1 0 50 0 0 12 0.0000 2 195 1410 11565 2610 of $\\tilde{x}[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4185 3465 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4635 3465 $+\\!4$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5085 3465 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5985 3465 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6885 3465 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5535 3465 $+\\!6$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6435 3465 $+\\!8$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8235 3465 $+\\!12$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7335 3465 $+\\!10$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7785 3465 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8685 3465 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9135 3465 $+\\!14$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9585 3465 $+\\!15$\001
4 1 0 50 0 0 12 0.0000 2 195 660 2025 3465 $y[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 2700 3465 $y[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 3510 3465 $y[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 195 1125 10305 3465 $y[k_0\\!+\\!16]$\001
4 1 0 50 0 0 12 0.0000 2 195 660 2025 1620 $x[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 2700 1620 $x[k_0\\!+\\!1]$\001
4 1 0 50 0 0 12 0.0000 2 195 1035 3510 1620 $x[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4185 1620 $+\\!3$\001
4 1 0 50 0 0 12 0.0000 2 165 465 4635 1620 $+\\!4$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5085 1620 $+\\!5$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5985 1620 $+\\!7$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6885 1620 $+\\!9$\001
4 1 0 50 0 0 12 0.0000 2 165 465 5535 1620 $+\\!6$\001
4 1 0 50 0 0 12 0.0000 2 165 465 6435 1620 $+\\!8$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8235 1620 $+\\!12$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7335 1620 $+\\!10$\001
4 1 0 50 0 0 12 0.0000 2 165 555 7785 1620 $+\\!11$\001
4 1 0 50 0 0 12 0.0000 2 165 555 8685 1620 $+\\!13$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9135 1620 $+\\!14$\001
4 1 0 50 0 0 12 0.0000 2 165 555 9585 1620 $+\\!15$\001
4 1 0 50 0 0 12 0.0000 2 195 1125 10305 1620 $x[k_0\\!+\\!16]$\001
4 1 0 50 0 0 12 0.0000 2 195 1215 2025 765 $\\tilde{x}[k_0]$\001
4 1 0 50 0 0 12 0.0000 2 195 1500 5535 765 $\\hat{x}[k_0\\!+\\!6]$\001
4 1 0 50 0 0 12 0.0000 2 195 1500 6435 765 $\\hat{x}[k_0\\!+\\!8]$\001
4 1 0 50 0 0 12 0.0000 2 165 285 4500 3870 $L$\001
4 1 0 50 0 0 12 0.0000 2 165 285 8685 3870 $L$\001
4 1 0 50 0 0 12 0.0000 2 135 675 900 2790 available\001
4 1 0 50 0 0 12 0.0000 2 195 1500 3510 765 $\\hat{x}[k_0\\!+\\!2]$\001
4 1 0 50 0 0 12 0.0000 2 180 1365 4635 5220 Complete diagram\001


==> Pic/simresults <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
0 32 #000000
0 33 #dcdcdc
0 34 #b5b5b5
6 7600 8125 7690 8215
2 1 0 1 1 7 49 0 41 0.000 0 0 -1 0 0 2
	 7600 8125 7690 8215
2 1 0 1 1 7 49 0 41 0.000 0 0 -1 0 0 2
	 7600 8215 7690 8125
-6
2 5 0 1 0 -1 50 0 -1 0.000 0 0 -1 0 0 5
	0 plot_paper.eps
	 4410 7740 12205 7740 12205 13836 4410 13836 4410 7740
2 2 0 1 7 7 50 0 41 0.000 0 0 -1 0 0 5
	 7470 8100 7830 8100 7830 8280 7470 8280 7470 8100
4 0 7 50 0 0 12 0.0000 2 195 270 6005 8525 $g$\001


==> Pic/sysmod <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
0 32 #000000
0 33 #dcdcdc
0 34 #b5b5b5
2 2 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4050 900 6300 900 6300 2250 4050 2250 4050 900
4 1 0 50 0 0 18 0.0000 2 195 1725 5175 1440 Linear Prefilter\001

